Type-Confusion Security

Type systems are a lightweight way to obtain formal assurance that code upholds security properties. However, decentralized systems, such as smart contracts and Model Context Protocol ecosystems, have limited ability to constrain the behavior of untrusted code. In such systems, attackers may attempt to confuse trusted code by supplying values that do not behave according to their advertised types, an attack that we call type confusion. Well-known attacks such as confused deputy attacks, reentrancy attacks, and control-flow hijacking can be understood as instances of type confusion. We define type confusion security as the property that unrestricted attackers who need not follow the type system have no more power than limited attackers who fully obey it. We formally define type confusion security as a real--ideal emulation, and in the context of an information-flow-typed core calculus that statically enforces security against well-typed attackers, prove that its run-time checks also enforce security against ill-typed attackers. In this system, programmers can write code while reasoning about security only against well-typed attackers; the security guarantees enforced by the type system still hold. We mechanize a proof of type confusion security in Lean.

==> paperversions.tex <==
\RequirePackage{paperversions}

